Learning Robust Visual-semantic Mapping for Zero-shot Learning

Zero-shot learning (ZSL) aims at recognizing unseen class examples (e.g., images) with knowledge transferred from seen classes. This is typically achieved by exploiting a semantic feature space shared by both seen and unseen classes, e.g., attributes or word vectors, as the bridge. In ZSL, the common practice is to train a mapping function between the visual and semantic feature spaces with labeled seen class examples. When inferring, given unseen class examples, the learned mapping function is reused to them and recognizes the class labels on some metrics among their semantic relations. However, the visual and semantic feature spaces are generally independent and exist in entirely different manifolds. Under such a paradigm, the ZSL models may easily suffer from the domain shift problem when constructing and reusing the mapping function, which becomes the major challenge in ZSL. In this thesis, we explore effective ways to mitigate the domain shift problem and learn a robust mapping function between the visual and semantic feature spaces. We focus on fully empowering the semantic feature space, which is one of the key building blocks of ZSL. In summary, this thesis targets fully empowering the semantic feature space and design effective solutions to mitigate the domain shift problem and hence obtain a more robust visual-semantic mapping function for ZSL. Extensive experiments on various datasets demonstrate the effectiveness of our proposed methods.

==> Publications.tex <==
\chapter{List of Publications}\label{ch:publications} 

$*$ indicates equal contribution (co-first authors)

\begin{itemize}

\item [11. ]
  \textbf{Jingcai Guo}, Shiheng Ma, Yuxia Sun and Song Guo, \textit{``Conservative Novelty Synthesizing Networks for Malware Recognition in an Open-set Scenario''}, submitted to \textit{IEEE Transactions on Neural Networks and Learning Systems (TNNLS)}, 2020.
  
  \item [10. ]
  Shiheng Ma$^{*}$, \textbf{Jingcai Guo$^{*}$}, Yuxia Sun, Song Guo and Minyi Guo, \textit{``A Multimodal Dual-Embedding Approach for Malware Open-set Recognition''}, submitted to \textit{Transactions on Emerging Topics in Computing (TETC)}, 2020.
  
  \item [9. ] 
  Qihua Zhou, Zhihao Qu, Song Guo, Boyuan Luo, \textbf{Jingcai Guo}, Zhenda Xu and Rajendra Akerkar, \textit{``On-device Learning Systems for Edge Intelligence: A Software and Hardware Synergy Perspective''}, submitted to \textit{IEEE Internet of Things Journal (IoTJ)}, 2020.
  
  \item [8. ] 
  \textbf{Jingcai Guo}, Song Guo and Jingya Wang, \textit{``Graph Knows Unknowns: Zero-shot Learning as a Graph Recognition''}, submitted to The \textit{34th Conference on Neural Information Processing Systems (NeurIPS)}, 2020.
     
  \item [7. ]
  \textbf{Jingcai Guo}, Shiheng Ma, Jie Zhang, Qihua Zhou and Song Guo, \textit{``Dual-view Attention Networks for Single Image Super-Resolution''}, The 28th \textit{ACM International Conference on Multimedia (ACM MM)}, 2020.
  
  \item [6. ]
  \textbf{Jingcai Guo} and Song Guo, \textit{``A Novel Perspective to Zero-shot Learning: Towards an Alignment of Manifold Structures via Semantic Feature Expansion''}, \textit{IEEE Transactions on Multimedia (TMM)}, 2020.
  
  \item [5. ] 
  \textbf{Jingcai Guo} and Song Guo, \textit{``Adaptive Adjustment with Semantic Feature Space for Zero-Shot Recognition''}, The \textit{44th IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP)}, 2019.
     
  \item [4. ]
   \textbf{Jingcai Guo} and Song Guo, \textit{``EE-AE: An Exclusivity Enhanced Unsupervised Feature Learning Approach''}, The \textit{44th IEEE International Conference on Acoustics, Speech, and Signal Processing (ICASSP)}, 2019.
  
  \item [3. ]
   \textbf{Jingcai Guo} and Song Guo, \textit{``AMS-SFE: Towards an Alignment of Manifold Structures via Semantic Feature Expansion for Zero-shot Learning''}, The \textit{20th IEEE International Conference on Multimedia and Expo (ICME)}, 2019.
  
  \item [2. ] 
  Shiheng Ma, \textbf{Jingcai Guo}, Song Guo and Minyi Guo, \textit{``Position-Aware Convolutional Networks for Traffic Prediction''}, \textit{ArXiv Technical Report, arXiv:1904.06187}, 2019.
     
  \item [1. ]
  \textbf{Jingcai Guo}, \textit{``An improved incremental training approach for large scaled dataset based on support vector machine''}, The \textit{3rd IEEE/ACM International Conference on Big Data Computing, Applications and Technologies (BDCAT)}, 2016.
  
 \end{itemize}





